Aircraft Collision Avoidance Systems: Technological Challenges and Solutions on the Path to Regulatory Acceptance

Aircraft collision avoidance systems is critical to modern aviation. These systems are designed to predict potential collisions between aircraft and recommend appropriate avoidance actions. Creating effective collision avoidance systems requires solutions to a variety of technical challenges related to surveillance, decision making, and validation. These challenges have sparked significant research and development efforts over the past several decades that have resulted in a variety of proposed solutions. This article provides an overview of these challenges and solutions with an emphasis on those that have been put through a rigorous validation process and accepted by regulatory bodies. The challenges posed by the collision avoidance problem are often present in other domains, and aircraft collision avoidance systems can serve as case studies that provide valuable insights for a wide range of safety-critical systems.

==> cas_policy_slices.tex <==
\begin{tikzpicture}[]
\begin{groupplot}[group style={horizontal sep=1cm, group size=2 by 1}]

\nextgroupplot [
% \begin{axis} [
  height = {5cm},
  ylabel = {$h$ (m)},
  title = {$\dot h_0 = \SI{0}{\meter\per\second}$},
  xmin = {0},
  xmax = {40},
  ymax = {400},
  xlabel = {$\tau$ (s)},
  x dir = reverse, 
  xtick pos=left, ytick pos=left, clip=false, 
  legend columns=3, legend style={at={(2.1, 1.4)}, draw=none, fill=none, font=\footnotesize, /tikz/every even column/.append style={column sep=0.5cm}}, legend image post style={scale=1.0},
  ymin = {-400},
  width = {5cm},
  enlargelimits = false,
  axis on top
]

\addlegendimage{area legend, fill=white};

\addlegendentry{no advisory};

\addlegendimage{area legend, fill=pastelGreen};

\addlegendentry{descend};

\addlegendimage{area legend, fill=pastelBlue};

\addlegendentry{climb};

\addplot+[
  point meta min = 1,
  point meta max = 3
] graphics[
  xmin = 0,
  xmax = 40,
  ymin = -400,
  ymax = 400
] {tmp_10000000000054.png};

\node [aircraft side,fill=pastelRed,minimum width=0.5cm,xscale=-1] at (axis cs: 0,0) {};;


\nextgroupplot [
  height = {5cm},
  title = {$\dot h_0 = \SI{4}{\meter\per\second}$},
  xmin = {0},
  xmax = {40},
  ymax = {400},
  xlabel = {$\tau$ (s)},
  x dir = reverse, xtick pos=left, ytick pos=left, clip=false, legend style={at={(0.8, 1)}, draw=none, fill=none, font=\tiny}, legend image post style={scale=0.5}, yticklabels={},
  ymin = {-400},
  width = {5cm},
  enlargelimits = false,
  axis on top
]

\addplot[
  point meta min = 1,
  point meta max = 3
] graphics[
  xmin = 0,
  xmax = 40,
  ymin = -400,
  ymax = 400, 
] {tmp_10000000000055.png};

\node [aircraft side,fill=pastelRed,minimum width=0.5cm,xscale=-1] at (axis cs: 0,0) {};;


\end{groupplot}

\end{tikzpicture}


